CHANG-ES XXXIX. Magnetic field structure in edge-on galaxies: Stacking Stokes parameters

Galactic magnetic fields regulate star formation and cosmic-ray (CR) transport, and understanding their three-dimensional structure, particularly in star-forming late-type galaxies, is key to constraining galactic CR transport. We explore the validity of stacking Stokes $Q$ and $U$ spectra, to infer about the intrinsic polarisation characteristics of star-forming galaxies. To prepare the stacking experiment, we align, scale, convolve, and reproject $C$-band (6 GHz) Stokes $Q$ and Stokes $U$ cubes of 27 star-forming late-type edge-on galaxies. On the stacked cubes, we perform RM-synthesis and discuss the derived polarised intensity (PI), polarisation angle ($\chi_0$), and RM maps. Synthetic data tests demonstrate that stacking Stokes $Q$ and $U$ spectra is valid for tightly constrained underlying distributions of PI, $\chi_0$, and RM. For underlying PI, $\chi_0$, and RM distributions that represent star-forming galaxies, stacking introduces a systematic uncertainty of $\delta_\mathrm{RM}^\mathrm{sys}=90 \mathrm{rad m^{-2}}$ and significantly underestimates the recovered PI. Stacking results reveal a clear X-shaped pattern in the polarisation plane, consistent with prior findings, detecting polarised emission up to 9 kpc above the galactic disc. We find stronger PI on the approaching side of galaxies. Furthermore, we find a decrease in PI in the galactic halo of $\sim 60$% near the galaxy's minor axis. A global RM pattern, as reported in a previous study, cannot be confirmed. Based on our analysis, we present stacking of Stokes $Q$ and Stokes $U$ cubes as an effective tool to recover faint polarised emission in the halo of nearby galaxies, if the underlying distributions of PI, $\chi_0$, and RM are tightly constrained. Our findings motivate future studies using broader-band data to increase the resolution in Faraday depth.

==> variables.tex <==
\newcommand{\nstackang}{21}
\newcommand{\angstackminsampling}{15.0}
\newcommand{\regridnpixang}{150.0}
\newcommand{\angstackinnerradiusbeams}{2.5}
\newcommand{\angstackouterradiusbeams}{7.5}
\newcommand{\beampixratioangular}{5.0}
\newcommand{\rmnormval}{50}
\newcommand{\rmminnpix}{10}
\newcommand{\phyres}{2}
\newcommand{\phypixsize}{0.4}
\newcommand{\phyrefdistance}{20}

